Sentence Embedding Leaks More Information than You Expect: Generative Embedding Inversion Attack to Recover the Whole Sentence

Sentence-level representations are beneficial for various natural language processing tasks. It is commonly believed that vector representations can capture rich linguistic properties. Currently, large language models (LMs) achieve state-of-the-art performance on sentence embedding. However, some recent works suggest that vector representations from LMs can cause information leakage. In this work, we further investigate the information leakage issue and propose a generative embedding inversion attack (GEIA) that aims to reconstruct input sequences based only on their sentence embeddings. Given the black-box access to a language model, we treat sentence embeddings as initial tokens' representations and train or fine-tune a powerful decoder model to decode the whole sequences directly. We conduct extensive experiments to demonstrate that our generative inversion attack outperforms previous embedding inversion attacks in classification metrics and generates coherent and contextually similar sentences as the original inputs.

==> app-tab-decode.tex <==
%\begin{table*}[!htbp]
\begin{sidewaystable*}
%\begin{table*}[t]
\centering
\small
  \begin{tabular}{c l c  cccccc  ccc  ccc ccc}
    \toprule
    \multirow{2}{*}{Data} &
    \multirow{2}{*}{Victim Model} &
    \multicolumn{1}{c}{\multirow{2}{*}{Decode}} &
    \multicolumn{1}{c}{\multirow{2}{*}{PPL}} &
    \multicolumn{1}{c}{\multirow{2}{*}{ES}} &
      \multicolumn{2}{c}{ROUGE} &
      \multicolumn{3}{c}{BLEU} &
      \multicolumn{3}{c}{Classification} &
      \multicolumn{1}{c}{\multirow{2}{*}{EMR}} &
      \multicolumn{2}{c}{ED} &
       \\
      {} & {} & {} & {} & {} & {ROUGE-1} & {ROUGE-L} & {BLEU-1} & {BLEU-2} & {BLEU-4} & Pre & Rec & F1 & {} & Mean & Median\\
      \midrule
      \multirow{10}{*}{PC} 
    & SRoBERTa        & & 7.52 & 83.77 & 44.55 & 41.00 & 30.16 & 13.31 & 9.75 & 39.60 & 39.54 & 39.57 & 8.71 & 33.10 & 35\\
    %\hline
    & SimCSE-BERT     & & 8.70 & 86.56 & 54.83 & 48.94 & 38.24 & 19.01 & 14.15 & 46.81 & 47.24 & 47.03  & 11.05 & 31.16 & 32 \\
    & SimCSE-RoBERTa  & Nucleus & 8.46 & 86.48 & 50.56 & 44.90 & 35.20 & 16.04 & 11.53 & 44.09 & 44.13 & 44.11 & 8.43 & 32.63 & 34 \\
    & ST5             & & 8.45 & 88.31 & 55.55 &  50.21 & 38.42 & 19.18 & 14.29 & 48.42 & 48.32 & 48.37 & 11.54 & 29.83 & 31 \\
    & MPNet           & & 8.30 & 85.88 & 50.49 & 45.88 & 34.53 & 16.21 & 12.03 & 44.32 & 44.31 & 44.32 & 10.44 & 31.45 & 33 \\
    
    \cmidrule(lr){2-17}
    %\midrule  %%%%% PC beam search decoding is used here
    & SRoBERTa        & & 4.78 & 85.81 & 50.68 & 47.30 & 31.62 & 16.19 & 12.22 & 47.92 & 42.65 & 45.13 & 10.40 & 29.63 & 30 \\
    %\hline
    & SimCSE-BERT     & & 6.68 & 88.23 & 60.02 & 54.09 & 41.02 & 22.25 & 16.85 & 52.52 & 50.88 & 51.69 & 12.99 & 28.43 & 29 \\
    & SimCSE-RoBERTa  & Beam & 5.33 & 88.19 & 56.45 & 51.10 & 36.22 & 18.84 & 14.01 & 51.86 & 46.78 & 49.19 & 10.43 & 28.95 & 30 \\
    & ST5             & & 5.50 & 90.26 & 62.18 & 57.11 & 40.10 & 22.84 & 17.53 & 57.20 & 51.69 & 54.31 & 14.48 & 26.15 & 26 \\
    & MPNet           & & 5.39 & 87.89 & 56.82 & 52.38 & 36.21 & 19.56 & 14.90 & 52.78 & 47.68 & 50.10 & 12.69 & 27.87 & 28 \\
    \midrule
    \midrule  %%%%% sampling decoding for qnli
    \multirow{10}{*}{QNLI} 
    & SRoBERTa        & & 25.48 & 80.13 & 26.65 & 22.45 & 20.32 & 3.95 & 2.47 & 28.40 & 27.09 & 27.73 & 0.17 & 95.99 & 75 \\
    %\hline
    & SimCSE-BERT     & & 26.36 & 80.45 & 30.71 & 26.22 & 23.03 & 5.21 & 3.50 & 30.27 & 29.07 & 29.66 & 0.21 & 91.21 & 70 \\
    & SimCSE-RoBERTa  & Nucleus & 22.85 & 80.13 & 27.85 & 23.76 & 20.54 & 4.26 & 2.75 & 29.12 & 27.26 & 28.16 & 0.22 & 94.97 & 74 \\
    & ST5             & & 28.74 & 83.21 & 32.77 & 27.86 & 24.11 & 5.86 & 3.91 & 31.84 & 30.69 & 31.25 & 0.37 & 90.71 & 71 \\
    & MPNet           & & 28.66 & 81.46 & 29.94 & 25.11 & 22.57 & 4.88 & 3.19 & 30.38 & 29.23 & 29.80 & 0.33 & 93.72 & 74 \\
    
    \cmidrule(lr){2-17}
    %\midrule  %%%%% beam search decoding for qnli
    & SRoBERTa        & & 11.09 & 81.18 & 30.54 & 26.23 & 20.40 & 4.97 & 3.28 & 35.02 & 27.33 & 30.70 & 0.32 & 87.47 & 67 \\
    %\hline
    & SimCSE-BERT     & & 11.74 & 81.37 & 34.24 & 29.83 & 22.63 & 6.24 & 4.35 & 36.84 & 28.87 & 32.37 & 0.50 & 84.77 & 65 \\
    & SimCSE-RoBERTa  & Beam & 10.43 & 81.34 & 31.69 & 27.46 & 20.50 & 5.27 & 3.53 & 35.69 & 27.47 & 31.04 & 0.41 & 87.13 & 67 \\
    & ST5             & & 12.06 & 84.15 & 36.58 & 31.75 & 23.31 & 6.82 & 4.70 & 39.05 & 30.30 & 34.13 & 0.75 & 83.79 & 64 \\
    & MPNet           & & 12.59 & 82.52 & 33.88 & 28.92 & 22.21 & 5.84 & 3.94 & 37.18 & 29.23 & 32.73 & 0.58 & 85.97 & 66 \\

    \bottomrule
  \end{tabular}
  \vspace{-0.05in}
  \caption{\label{tab:decode methods}
A complete evaluation of generation quality with different decoding algorithms.
EMR refers to the exact match ratio and ED stands for the edit distance.
Embedding Similarity, ROUGE, BLEU, Pre, Rec, F1 and EMR are measured in \%.
To make inverted results close to the original inputs, a smaller ED with a larger EMR is expected for embedding inversion attacks.
}
\vspace{-0.05in}
%\end{table*}
\end{sidewaystable*}






==> app-tab-domain.tex <==
\begin{table*}[t]
\centering
\small
  \begin{tabular}{c l  c cc ccc  ccc }
    \toprule
    \multirow{2}{*}{} &
    \multirow{2}{*}{Victim} &
    \multirow{2}{*}{ES} &
      \multicolumn{2}{c}{ROUGE} &
      \multicolumn{2}{c}{BLEU} &
      \multicolumn{3}{c}{Classification} &
      \multicolumn{1}{c}{\multirow{2}{*}{EMR}} 
       \\
      {} & {} & {} & {ROUGE-1} & {ROUGE-L} & {BLEU-1} & {BLEU-4} & Pre & Rec & F1 & {}\\
      \midrule
      \multirow{5}{*}{\shortstack{PC \\ to \\ QNLI}} 
     & SRoBERTa                 & 67.39 & 11.66 & 10.14 & 6.25 & 0.14 & 21.66 & 12.44 & 15.80 & 0 \\ %& 24.83 & 24\\
     & SimCSE-BERT              & 72.28 & 21.76 & 18.96 & 10.58 & 0.75 & 29.62 & 18.21 & 22.55 & 0 \\ %& 26.15 & 26\\
     & SimCSE-RoBERTa           & 71.27 & 19.51 & 17.35 & 7.24 & 0.62 & 31.08 & 15.32 & 20.52 & 0 \\ %& 25.35 & 25\\
     & ST5                      & 73.60 & 20.80 & 17.95 & 8.85 & 0.68 & 30.25 & 16.50 & 21.35 & 0 \\ %& 25.56 & 25\\
     & MPNet                    & 69.81 & 15.42 & 13.35 & 7.66 & 0.39 & 23.94 & 14.66 & 18.18 & 0 \\ %& 25.56 & 25\\
     
     \midrule
     \midrule
      \multirow{5}{*}{\shortstack{QNLI \\ to \\ PC}} 
     & SRoBERTa                 & 67.88 & 8.54 & 7.43 & 5.23 & 0.11 & 9.27 & 16.98 &11.99 & 0 \\ %& 24.83 & 24\\
     & SimCSE-BERT              & 72.82 & 21.77 & 19.24 & 12.08 & 1.32 & 21.69 & 20.63 & 21.15 & 0 \\ %& 26.15 & 26\\
     & SimCSE-RoBERTa           & 71.53 & 17.63 & 15.47 & 10.90 & 0.84 & 18.63 & 19.08 & 18.85 & 0 \\ %& 25.35 & 25\\
     & ST5                      & 74.00 & 18.45 & 16.14 & 10.89 & 0.90 & 20.14 & 19.57 & 19.85 & 0 \\ %& 25.56 & 25\\
     & MPNet                    & 71.25 & 14.17 & 12.26 & 8.60 & 0.53 & 14.02 & 18.69 & 16.02 & 0 \\ %& 25.56 & 25\\


    \bottomrule
  \end{tabular}
  \vspace{-0.05in}
  \caption{\label{tab:domain adaption}
Evaluation results on domain adaptation.
}
\vspace{-0.05in}
\end{table*}

==> tab-performance.tex <==

\begin{table*}[!htbp]
%\begin{adjustbox}{angle=90}
\centering
\small
  \begin{tabular}{l  cccccc | ccccc}
    \toprule
    \multirow{2}{*}{} &
%    \multicolumn{1}{c}{\multirow{2}{*}{PPL}} &
      \multicolumn{6}{c|}{Multi-label Classification} &
      \multicolumn{5}{c}{Improved Embedding Inversion} \\
      & {Threshold} & {Pre} & {Rec} & {F1} & {NERR} & {SWR} & {Pre} & {Rec} & {F1} & {NERR} & {SWR} \\
      \midrule
    SRoBERTa        & 0.2 & 33.42 & 26.79 & 29.74 & 0.00053 & 0.999 & 39.60 & 39.54 & 39.57 & 0.17 & 0.545 \\
    %\hline
    SimCSE-BERT     & 0.5 & 24.77 & 21.36 & 22.94 & 0.00026 & 0.406 & 46.81 & 47.24 & 47.03& 0.33 & 0.528\\
    SimCSE-RoBERTa  & 0.5 & 54.58 & 28.15 & 37.14 & 0.0087 & 0.616& 44.09 & 44.13 & 44.11 & 0.27 & 0.540\\
    ST5             & 0.1 & 22.93 & 38.17 &  28.65 & 0.00053 & 0.947 & 48.42 & 48.32 & 48.37 & 0.28 & 0.539\\
    MPNet           & 0.2 & 33.91 & 27.39 & 30.30 & 0.00053 & 0.999 & 44.32 & 44.31 & 44.32 & 0.21 & 0.539\\
    \bottomrule
  \end{tabular}
  %\end{adjustbox}
  \vspace{-0.05in}
  \caption{\label{tab:performance}
Embedding inversion performance comparison between Multi-label Classification and improved embedding inversion on classification metrics. 
The token-level micro-averaged precision, recall and F1 are reported.
Precision (Pre), recall (Rec), F1, NERR and SWR are measured in \%.
To study whether the inverted tokens are sensitive or not, we also evaluate on the named entity recovery ratio (NERR) and stopword rate (SWR).
High Pre, Rec and F1 indicates good attacking performance on classification.
High NERR with low SWR suggests that the recovered tokens are informative while high SWR with low NERR indicates that the attack is not harmful despite good classification performance.
}

%\vspace{-0.05in}
\end{table*}


